Sequential importance sampling for estimating expectations over the space of perfect matchings

This paper makes three contributions to estimating the number of perfect matching in bipartite graphs. First, we prove that the popular sequential importance sampling algorithm works in polynomial time for dense bipartite graphs. More carefully, our algorithm gives a $(1\pm\epsilon)$-approximation for the number of perfect matchings of a $\lambda$-dense bipartite graph, using $O(n^{\frac{1-2\lambda}{\lambda}\epsilon^{-2}})$ samples. With size $n$ on each side and for $\frac{1}{2}>\lambda>0$, a $\lambda$-dense bipartite graph has all degrees greater than $(\lambda+\frac{1}{2})n$. Second, practical applications of the algorithm require many calls to matching algorithms. A novel preprocessing step is provided which makes significant improvements. Third, three applications are provided. The first is for counting Latin squares, the second is a practical way of computing the greedy algorithm for a card-guessing game with feedback, and the third is for stochastic block models. In all three examples, sequential importance sampling allows treating practical problems of reasonably large sizes.

==> card_guessing.tex <==

In this section, we apply the repeated estimation of the number of matchings in bipartite graphs to a card guessing experiment. The card guessing experiment starts 
with a well shuffled deck of $N$ cards. A subject guesses the cards one at a time, sequentially, going through the deck. After each guess, the subject is told if their guess is correct or wrong. 

Card guessing experiments with feedback occur in Fisher's tasting tea \cite{fisher:1935}, in evaluation of randomized clinical trials \cite{BlackwellHodges, EfronClinicalTrial}, in ESP experiments \cite{DiaconisESPsearch}, and in optimal strategy in casino card games such as blackjack or baccarat \cite{ethier_levin_2005}. A review is in \cite{DiaconisCompleteFeedback,DiaconisGrahamHolmes}. The recent papers \cite{diaconis2020card,diaconis2020guessing} developed practical  strategies which do perform close to optimal and gave bounds on the expected score under the optimal strategy.

Given a shuffled deck of cards, how should the subject use the feedback to get a high score? 
Extensive numerical work in the literature suggests that greedy (guessing the most likely card given the feedback) is close to optimal. Next we will see that implementing the greedy strategy reduces to evaluating the permanent of a matrix. Then we apply SIS to estimate the expected number of correct guesses using  the greedy strategy for any reasonable deck size. The exact value of greedy was only known for small decks in the literature, and the SIS estimator is close to the known exact values.



To see the relation of card guessing experiments and evaluating permanents let us fix some notation. Consider a deck of $N$ cards, with $d$ distinct values (say, $1, 2, \ldots, d
$) with value $i$ repeated $k_i$ times, so $\sum_1^d k_i = N$. An example is a normal deck of cards $(N = 52)$ with $13$ values each with multiplicity $4$. 

The deck is shuffled and a guessing subject makes sequential guesses. Each time the subject is told if the guess is correct or not. { Consider we want to find the card that the greedy strategy chooses for the next step. Let $a_i$ be the number of cards labeled $i$ that have been in the deck so far but the guessing subject has not guessed them correctly. }
% Consider the situation that there are $a_i$ cards labeled $i$ that are not guessed yet. 
Moreover, let $b_i$ be the number of incorrect guesses where the subject chose card labeled $i$.  As a consequence of the definitions, $\sum_{i=1}^d a_i= \sum_{i=1}^d b_i$.
Let $N(a,b)$ be the number of permutations of a deck of $N' = \sum_1^d a_i$ cards, where cards labeled $1$ are not in first $b_1$ positions and cards labeled $2$ are not in next $b_2$ positions and so on.
Then $N(a,b) = \per(M_{ab})$ with  $M_{ab}$ a zero-one matrix with zero blocks of size $a_1\times b_1,a_2\times b_2,\ldots$ as shown in Figure \ref{fig:zero_block_matrix}.
\begin{figure}[htbp]
\begin{center}
  \includegraphics[scale=0.35]{images/zero_block_matrix.png}
  \caption{An example of structure of card guessing matrix ($M_{ab}$).}
  \label{fig:zero_block_matrix}
\end{center}
\end{figure}

The number of consistent arrangements with card labeled $i$ in the next position is equal $N(a^{*i},b)$ where $a^{*i}_i = a_i - 1$ and $a^{*i}_j = a_j$ for all $j \neq i$. Thus, the chance that next guess is $i$ equals
$$\frac{N(a^{*i},b)}{N(a,b)}.$$ 
The greedy algorithm guesses $i$ to maximize this ratio. Naively, $d$ permanents must be evaluated at each stage. Some theory allows a simplification. In \cite{ChungPermanent}, the following theorem is proved.
\begin{theorem}\label{thm: greedy alg}
With Yes/No feedback, following an incorrect guess of $i$, the greedy strategy is to guess $i$ for the next guess.
\end{theorem}




Theorem~\ref{thm: greedy alg} shows that the permanent must only be evaluated following a correct guess. Our algorithm for card guessing use the sequential importance sampling algorithm developed in the sections above to do this via Monte Carlo: fix $B$ and generate random matchings in the appropriate bipartite graph $B$ times, weighting each matching by its probability. Use these weighted samples to estimate the chance that the next card is $i$ and choose the maximizing $i^*$.


Throughout, we simulate greedy using `guess card $i$ until told correct' to start. After a `Yes' answer, sequential importance sampling  runs $B$ times as above to estimate the chance of the $d$ possible values for the next card. The most probable is chosen and one keeps guessing this value until `Yes'. Then again begins to simulate, and repeats the procedure above. The plots below compare various values of $B$.

\textbf{ Example 1 ($k=2$ and varying $d$):}
We begin by discussing a long open case. A deck of size $2d$ of composition $1,1,2,2,3,3,\ldots,d,d$. It was open until recently whether the expected number of correct guesses is unbounded in $d$. In \cite{diaconis2020card} it was shown to be bounded by $6$ for all $d$. %In \cite{diaconis2020guessing} a variant of guess $1$, then $2, \ldots$, was proved to have expectation more than $2.91.$ 
Figure \ref{fig: k=2 guess card} shows some numbers.

\begin{figure}[htbp]
\begin{center}
  \includegraphics[scale=0.19]{images/Figure_m2.jpg}
  \caption{Comparison between different algorithms when $k=2$. The $95\%$ confidence intervals are highlighted.}\label{fig: k=2 guess card}
\end{center}
\end{figure}


\begin{remark}
The figure shows estimates of the expected values with $B=100$ and $B=1000$. The shaded regions are pointwise $95\%$ confidence intervals. Averages are based on $10000$ repetitions. These figures suggest that the lower bound $2.91$ from \cite{diaconis2020guessing} is close to the truth.
\end{remark}
The exact computation of general permanents is a well-known $\#P$-complete problem. However, on reflection, we have found that the permanents of matrices of the form of Figure \ref{fig:zero_block_matrix} can be exactly computed; in linear time in the size of the matrix (see Appendix \ref{sec: exact permanent card guessing}). Having an exact algorithm allows us to check the numerical examples for card guessing. For small values of $d$ the exact expectation of greedy expectations was computed by backward induction for $d=2,3,4,5$ in Table \ref{tab:guesses d=k} and for larger $d$, we use our exact greedy algorithm to estimate the greedy strategy. %Despite expectation, the values are not monotone increasing in $d$ as shown in Figure \ref{fig: k=2 guess card}.

\begin{table}[htbp]
    \centering
    \begin{tabular}{||c||c|c|c||}
    \hline
        $d$ & GREEDY & SIS with $B=100$ & SIS with $B=1000$\\
    \hline\hline
        $2$ & 2.8333 & \begin{tabular}{@{}c@{}}$2.8343$\\$(2.8265, 2.8421)$\end{tabular} & \begin{tabular}{@{}c@{}}$2.8338$\\$(2.8260, 2.8415)$\end{tabular}\\
        \hline
        $3$ & 3.0111 & \begin{tabular}{@{}c@{}}$3.0047$\\$(2.9937, 3.0158)$\end{tabular} & \begin{tabular}{@{}c@{}}$3.0074$\\$(2.9962, 3.0186)$\end{tabular}\\
        \hline
        $4$ & 3.0333 & \begin{tabular}{@{}c@{}}$3.0037$\\$(2.9912, 3.0162)$\end{tabular} & \begin{tabular}{@{}c@{}}$3.0164$\\$(3.0039, 3.0289)$\end{tabular}\\
        \hline
        $5$ & 3.0433 & \begin{tabular}{@{}c@{}}$3.0060$\\$(2.9930, 3.0190)$\end{tabular} & \begin{tabular}{@{}c@{}}$3.0162$\\$(3.0031, 3.0292)$\end{tabular}\\
        \hline
        $10$ & \begin{tabular}{@{}c@{}}$2.9786$\\$(2.9773, 2.9799)$\end{tabular} & \begin{tabular}{@{}c@{}}$2.9784$\\$(2.9649, 2.9918)$\end{tabular} & \begin{tabular}{@{}c@{}}$2.9741$\\$(2.9606, 2.9876)$\end{tabular}\\
        \hline
        $20$ & \begin{tabular}{@{}c@{}}$2.9585$\\$(2.9571, 2.9598)$\end{tabular} & \begin{tabular}{@{}c@{}}$2.9589$\\$(2.9454, 2.9724)$\end{tabular} & \begin{tabular}{@{}c@{}}$2.9557$\\$(2.9423, 2.9691)$\end{tabular}\\
        \hline
    \end{tabular}
    \caption{Greedy versus SIS estimator with $95\%$ confidence interval for $k=2$}
    \label{tab:guesses d=k}
\end{table}



\textbf{Example 2 ($d=k$)}: The classical ESP experiment had $d=k=5$. The theorems in \cite{diaconis2020card} and \cite{diaconis2020guessing} worked for fixed $k$ and large $d$ or fixed $d$ and large $k$. There are virtually no results for guesses when both $k$ and $d$ are large. Using SIS any reasonable deck sizes are now accessible. Fig. \ref{fig:CardGuessingM=n} shows results using sequential importance sampling for $d=k$ for $2 \leq d = k \leq 18$. The algorithm in Appendix \ref{sec: exact permanent card guessing} allows computing the number of correct guesses by the greedy algorithm for larger $d=k$. Note that the number of correct guesses by greedy depends on the order of the cards in the shuffled deck, and as a result we show confidence intervals both for greedy and SIS in Fig. \ref{fig:CardGuessingM=n}. 
\begin{figure}[htbp]
  \includegraphics[scale=0.16]{images/Figure_nm.jpg}
  \caption{Comparison between different algorithms when $d=k$. The $y$-axis represents 'the number of guessed cards'$-d$. The $95\%$ confidence intervals are highlighted.}\label{fig:CardGuessingM=n}
\end{figure}



\begin{remark}
From this data, the greedy algorithm guesses at least $d$ cards correctly. From previous data, it was not clear if the excess over $k$ even got as large as $2$ (!). We now believe that for $k=d$, the experiment of the greedy strategy is $d + \sqrt{d} + o(\sqrt{d})$ (see Fig. \ref{fig:nMinusSqrtn} ).
\end{remark}

\begin{figure}[htbp]
\begin{center}
  \includegraphics[scale=0.13]{images/nsqrtn.png}
  \caption{The plot of the `guessed cards' $- \sqrt{d}$ when $d=k$. The $95\%$ confidence intervals are  too narrow to present, with $(2.8213, 2.8484)$ for $d=2$ and $(66.5565, 67.2839)$ for $d=62$.}\label{fig:nMinusSqrtn}
\end{center}
\end{figure}



==> old_intro.tex <==


% main goal
Given a bipartite graph $G(X, Y)$ with $|X|=|Y|=n$, a perfect matching is a subgraph of $G$ in which all vertices have degree exactly one. We study the question of uniform sampling of perfect matchings in bipartite graphs. By the classical equivalences between approximate counting and sampling \cite{JERRUM1986169}, the study of sampling perfect matchings is equivalent to approximating the permanent of the adjacency matrix.

%permanents are hard but people used MCMC
Computing the permanent of an arbitrary $0-1$ matrix is $\#$P-complete \cite{VALIANT1979189}. In fact, the class of $\#$P-complete problems was introduced for the particular problem of computing permanent.
Despite the fact that there seems to be no algorithm for computing the permanent in the general case, when all the entries of the matrix is nonnegative real numbers there exists a fully polynomial randomized approximation scheme (FPRAS) \cite{Jerrum:2004:PAA:1008731.1008738}. This celebrated result is based on Markov Chain Monte Carlo (MCMC) methods where they use a general technique former designed by Broder to analyze the mixing time of an ergodic Markov chain \cite{SINCLAIR198993, Broder1986HowHI}.


% importance sampling as another method
In parallel to MCMC methods, importance sampling is another method to approximate the permanent. Diaconis and Kolesnik \cite{Diaconis2018SequentialIS,diaconis2019randomized}, analyzed an importance sampling algorithm as follows: First draw a uniform permutation $\pi$ over one side of the graph, $X$. Then iterate over the vertices in $X$ according to $\pi$, and in step $i$ match the vertex $\pi(i)$ with one of its neighbor in $Y$ (amongst the remaining allowable options), drawn uniformly at random. Diaconis and Kolesnik \cite{Diaconis2018SequentialIS,diaconis2019randomized} proved central limit theorems for the number of samples when input is Fibonacci permutations, a special case of ``interval" graphs in which the vertex $i$ in $X$ is adjacent to the vertices $[i-s,i+t]$ in $Y$ for some fixed $s, t\geq 0$. In a different work, permanents of more general classes of interval graphs have been studied by Tsao \cite{tsao2020theoretical}. 


%modification of the algorithm
Here, we use a similar algorithm. However, instead of drawing edges uniformly at random, we use the doubly stochastic scaling of the adjacency matrix to draw edges. See Algorithm  \ref{alg: SIS-matching}, which outputs a perfect matching along with the probability of sampling such matching.
We have two main theoretical contributions in this paper. First, we bound the number of samples needed for Algorithm \ref{alg: SIS-matching} to approximate the uniform distribution when the underlying graph is $\lambda$-dense, defined as follows. For some constant $\lambda>0$, the  bipartite graph $G(X,Y)$ with $|X|=|Y|=n$  is called  $\lambda$-dense if the degree of each vertex is at least $(\frac{1}{2}+\lambda)n$. 
Second, we give faster implementation of the algorithm in \cite{diaconis2019randomized} for sampling one perfect matching for general graphs (see Appendix \ref{sec: fast implmnt SIS}).

To state the main result, we need the following notation. For an adjacency matrix $A$, define its doubly-stochastic scaling $Q^A$, a matrix with row and column sums equal to $1$, which can be written as
\begin{equation}\label{eq: DS scaling}
    Q^A=D_\alpha A D_\beta,\qquad \text{$D_\alpha$ and $D_\beta$ are diagonal matrices.}
\end{equation}
 Let $(M_1,X_1),\ldots,(M_N,X_N)$ be the outputs of $N$ independent runs of Algorithm \ref{alg: SIS-matching} with $Q^A$ as an input, where $M_i$ is a perfect matching and $X_i$ is the probability of sampling $M_i$. To count the number of perfect matchings define the estimator as
\begin{equation}\label{eq: matching estimator}
I_N=\frac{1}{N}\sum_{i=1}^NX_i^{-1}.
\end{equation}


\begin{theorem} \label{thm: PTAS dense graph}
Given $\lambda>0$ let $G$ be a $\lambda$-dense graph of size $2n$. Also, let $M(G)$ be the number of perfect matchings in $G$. Then
Algorithm \ref{alg: SIS-matching} with $Q^A$ as an input, is a polynomial time approximation scheme (PTAS) for $M(G)$, i.e, given $\epsilon>0$, there exists a constant $C>0$ such that for $N\geq Cn^{\frac{1-2\lambda}{8\lambda}+\epsilon^{-2}}$, \[\mathbb{E}\left(\frac{|I_N-M(G)|}{M(G)}\right)\leq 3\epsilon.\]
\end{theorem}

%lit. rev. dense
 For a dense bipartite graphs, in which the degree of each vertex is more than $n/2$, Jerrum and Sinclair showed the running time of their algorithm to approximate permanent is $O(n^{10}\log(n)^3)poly\log(\epsilon^{-1})$, where $\epsilon$ is the total variation distance of the uniform distribution and their sampling distribution \cite{Jerrum:2004:PAA:1008731.1008738}. This was improved to $O(n^7\log(n)^4)$ by Bez\'{a}kov\'{a} \cite{bezakova}. Later an exact sampling algorithm for very dense graphs, where the degree of each vertex is at least $\lambda n$ for $\lambda>0.5$, was introduced in \cite{Huber-Law} based on rejection sampling, with the expected running time $O(n^4\log(n))$ for $\lambda\geq 0.6$. Their algorithm iterates over columns of the matrix  and chooses its match using a weaker version of Bregman-Minc inequality \cite{Bregman} to estimate the marginal probability of choosing a certain entry in each column. 

Here, we use the results by Chatterjee and Diaconis \cite{diaconis-chatterjee} to bound the number of samples in sequential importances algorithms. In general,  sequential importance sampling is used to   to approximate a complicated measure $\mu$ with a relatively simple measure $\nu$.
Chatterjee and Diaconis \cite{diaconis-chatterjee} characterized the necessary and sufficient number of samples by the KL-diveregence from $\nu$ to $\mu$, when $\log(d\nu/d\mu)$ is concentrated.  The main ingredient of proof of Theorem \ref{thm: PTAS dense graph} is to bound KL-divergence and use their result to find an upper bound on the number of samples.


\begin{remark}
Theorem \ref{thm: PTAS dense graph} bounds the number of samples needed by Algorithm \ref{alg: SIS-matching} with $Q^A$ as an input to approximate the number of perfect matchings in a $\lambda$-dense graph. Appendix \ref{sec:counter example matching} gives an example of graph with a bounded average degree that the original method of choosing edges uniformly at random in \cite{diaconis2019randomized} needs exponential number of samples, while using the doubly stochastic scaling will only need linear number of samples.
\end{remark}

Finally, we apply our algorithm to implement the greedy algorithm in card guessing experiments: A deck of $n$ cards is shuffled and then we have to guess the card on top of the deck sequentially. After each guess, we are told either our guess is wrong or right. Greedy algorithm is to guess most likely card at each step. While this algorithm is not optimal, it is known to be close to optimal. See \cite{diaconis2020card,diaconis2020guessing} for recent results on this topic.

Implementation of greedy needs approximating permanent of dense matrices repeatedly,for which we use Algorithm \ref{alg: SIS-matching}. Whereas the previous results could only approximate greedy for small decks, we are now able to apply the computations for decks of size $400$ (Figure \ref{fig:CardGuessingM=n}). 

%TODO add the latin square here

\subsection{Overview of the paper}
We start by going over some preliminaries on importance sampling in Section \ref{sec: prelim IS}. Then we proceed by proving Theorem \ref{thm: PTAS dense graph} in Section \ref{sec:dense}. The main idea is to bound the KL-divergence of the sampling distribution of Algorithm \ref{alg: SIS-matching}  with respect to the uniform distribution over the set of perfect matchings when the input matrix of the algorithm is the doubly stochastic scaling of the adjacency matrix.  Sections \ref{sec: experiment} and \ref{sec: latin square} is on the applications of our result to card guessing games and counting the number of Latin squares, respectively. 

==> sampling matching with importance sampling (Version 12917)/card_guessing.tex <==

In this section, we apply the repeated estimation of the number of matchings in bipartite graphs to a card guessing experiment. The card guessing experiment starts 
with a well shuffled deck of $N$ cards. A subject guesses the cards one at a time, sequentially, going through the deck. After each guess, the subject is told if their guess is correct or wrong. 

Card guessing experiments with feedback occur in Fisher's tasting tea \cite{fisher:1935}, in evaluation of randomized clinical trials \cite{BlackwellHodges, EfronClinicalTrial}, in ESP experiments \cite{DiaconisESPsearch}, and in optimal strategy in casino card games such as blackjack or baccarat \cite{ethier_levin_2005}. A review is in \cite{DiaconisCompleteFeedback,DiaconisGrahamHolmes}. The recent papers \cite{diaconis2020card,diaconis2020guessing} developed practical  strategies which do perform close to optimal and gave bounds on the expected score under the optimal strategy.

Given a shuffled deck of cards, how should the subject use the feedback to get a high score? 
Extensive numerical work in the literature suggests that greedy (guessing the most likely card given the feedback) is close to optimal. Next we will see that implementing the greedy strategy reduces to evaluating the permanent of a matrix. Then we apply SIS to estimate the expected number of correct guesses using  the greedy strategy for any reasonable deck size. The exact value of greedy was only known for small decks in the literature, and the SIS estimator is close to the known exact values.



To see the relation of card guessing experiments and evaluating permanents let us fix some notation. Consider a deck of $N$ cards, with $d$ distinct values (say, $1, 2, \ldots, d
$) with value $i$ repeated $k_i$ times, so $\sum_1^d k_i = N$. An example is a normal deck of cards $(N = 52)$ with $13$ values each with multiplicity $4$. 

The deck is shuffled and a guessing subject makes sequential guesses. Each time the subject is told if the guess is correct or not. { Consider we want to find the card that the greedy strategy chooses for the next step. Let $a_i$ be the number of cards labeled $i$ that have been in the deck so far but the guessing subject has not guessed them correctly. }
% Consider the situation that there are $a_i$ cards labeled $i$ that are not guessed yet. 
Moreover, let $b_i$ be the number of incorrect guesses where the subject chose card labeled $i$.  As a consequence of the definitions, $\sum_{i=1}^d a_i= \sum_{i=1}^d b_i$.
Let $N(a,b)$ be the number of permutations of a deck of $N' = \sum_1^d a_i$ cards, where cards labeled $1$ are not in first $b_1$ positions and cards labeled $2$ are not in next $b_2$ positions and so on.
Then $N(a,b) = \per(M_{ab})$ with  $M_{ab}$ a zero-one matrix with zero blocks of size $a_1\times b_1,a_2\times b_2,\ldots$ as shown in Figure \ref{fig:zero_block_matrix}.
\begin{figure}[htbp]
\begin{center}
  \includegraphics[scale=0.35]{images/zero_block_matrix.png}
  \caption{An example of structure of card guessing matrix ($M_{ab}$).}
  \label{fig:zero_block_matrix}
\end{center}
\end{figure}

The number of consistent arrangements with card labeled $i$ in the next position is equal $N(a^{*i},b)$ where $a^{*i}_i = a_i - 1$ and $a^{*i}_j = a_j$ for all $j \neq i$. Thus, the chance that next guess is $i$ equals
$$\frac{N(a^{*i},b)}{N(a,b)}.$$ 
The greedy algorithm guesses $i$ to maximize this ratio. Naively, $d$ permanents must be evaluated at each stage. Some theory allows a simplification. In \cite{ChungPermanent}, the following theorem is proved.
\begin{theorem}\label{thm: greedy alg}
With Yes/No feedback, following an incorrect guess of $i$, the greedy strategy is to guess $i$ for the next guess.
\end{theorem}




Theorem~\ref{thm: greedy alg} shows that the permanent must only be evaluated following a correct guess. Our algorithm for card guessing use the sequential importance sampling algorithm developed in the sections above to do this via Monte Carlo: fix $B$ and generate random matchings in the appropriate bipartite graph $B$ times, weighting each matching by its probability. Use these weighted samples to estimate the chance that the next card is $i$ and choose the maximizing $i^*$.


Throughout, we simulate greedy using `guess card $i$ until told correct' to start. After a `Yes' answer, sequential importance sampling  runs $B$ times as above to estimate the chance of the $d$ possible values for the next card. The most probable is chosen and one keeps guessing this value until `Yes'. Then again begins to simulate, and repeats the procedure above. The plots below compare various values of $B$.

\textbf{ Example 1 ($k=2$ and varying $d$):}
We begin by discussing a long open case. A deck of size $2d$ of composition $1,1,2,2,3,3,\ldots,d,d$. It was open until recently whether the expected number of correct guesses is unbounded in $d$. In \cite{diaconis2020card} it was shown to be bounded by $6$ for all $d$. %In \cite{diaconis2020guessing} a variant of guess $1$, then $2, \ldots$, was proved to have expectation more than $2.91.$ 
Figure \ref{fig: k=2 guess card} shows some numbers.

\begin{figure}[htbp]
\begin{center}
  \includegraphics[scale=0.19]{images/Figure_m2.jpg}
  \caption{Comparison between different algorithms when $k=2$. The $95\%$ confidence intervals are highlighted.}\label{fig: k=2 guess card}
\end{center}
\end{figure}


\begin{remark}
The figure shows estimates of the expected values with $B=100$ and $B=1000$. The shaded regions are pointwise $95\%$ confidence intervals. Averages are based on $10000$ repetitions. These figures suggest that the lower bound $2.91$ from \cite{diaconis2020guessing} is close to the truth.
\end{remark}
The exact computation of general permanents is a well-known $\#P$-complete problem. However, on reflection, we have found that the permanents of matrices of the form of Figure \ref{fig:zero_block_matrix} can be exactly computed; in linear time in the size of the matrix (see Appendix \ref{sec: exact permanent card guessing}). Having an exact algorithm allows us to check the numerical examples for card guessing. For small values of $d$ the exact expectation of greedy expectations was computed by backward induction for $d=2,3,4,5$ in Table \ref{tab:guesses d=k} and for larger $d$, we use our exact greedy algorithm to estimate the greedy strategy. %Despite expectation, the values are not monotone increasing in $d$ as shown in Figure \ref{fig: k=2 guess card}.

\begin{table}[htbp]
    \centering
    \begin{tabular}{||c||c|c|c||}
    \hline
        $d$ & GREEDY & SIS with $B=100$ & SIS with $B=1000$\\
    \hline\hline
        $2$ & 2.8333 & \begin{tabular}{@{}c@{}}$2.8343$\\$(2.8265, 2.8421)$\end{tabular} & \begin{tabular}{@{}c@{}}$2.8338$\\$(2.8260, 2.8415)$\end{tabular}\\
        \hline
        $3$ & 3.0111 & \begin{tabular}{@{}c@{}}$3.0047$\\$(2.9937, 3.0158)$\end{tabular} & \begin{tabular}{@{}c@{}}$3.0074$\\$(2.9962, 3.0186)$\end{tabular}\\
        \hline
        $4$ & 3.0333 & \begin{tabular}{@{}c@{}}$3.0037$\\$(2.9912, 3.0162)$\end{tabular} & \begin{tabular}{@{}c@{}}$3.0164$\\$(3.0039, 3.0289)$\end{tabular}\\
        \hline
        $5$ & 3.0433 & \begin{tabular}{@{}c@{}}$3.0060$\\$(2.9930, 3.0190)$\end{tabular} & \begin{tabular}{@{}c@{}}$3.0162$\\$(3.0031, 3.0292)$\end{tabular}\\
        \hline
        $10$ & \begin{tabular}{@{}c@{}}$2.9786$\\$(2.9773, 2.9799)$\end{tabular} & \begin{tabular}{@{}c@{}}$2.9784$\\$(2.9649, 2.9918)$\end{tabular} & \begin{tabular}{@{}c@{}}$2.9741$\\$(2.9606, 2.9876)$\end{tabular}\\
        \hline
        $20$ & \begin{tabular}{@{}c@{}}$2.9585$\\$(2.9571, 2.9598)$\end{tabular} & \begin{tabular}{@{}c@{}}$2.9589$\\$(2.9454, 2.9724)$\end{tabular} & \begin{tabular}{@{}c@{}}$2.9557$\\$(2.9423, 2.9691)$\end{tabular}\\
        \hline
    \end{tabular}
    \caption{Greedy versus SIS estimator with $95\%$ confidence interval for $k=2$}
    \label{tab:guesses d=k}
\end{table}



\textbf{Example 2 ($d=k$)}: The classical ESP experiment had $d=k=5$. The theorems in \cite{diaconis2020card} and \cite{diaconis2020guessing} worked for fixed $k$ and large $d$ or fixed $d$ and large $k$. There are virtually no results for guesses when both $k$ and $d$ are large. Using SIS any reasonable deck sizes are now accessible. Fig. \ref{fig:CardGuessingM=n} shows results using sequential importance sampling for $d=k$ for $2 \leq d = k \leq 18$. The algorithm in Appendix \ref{sec: exact permanent card guessing} allows computing the number of correct guesses by the greedy algorithm for larger $d=k$. Note that the number of correct guesses by greedy depends on the order of the cards in the shuffled deck, and as a result we show confidence intervals both for greedy and SIS in Fig. \ref{fig:CardGuessingM=n}. 
\begin{figure}[htbp]
  \includegraphics[scale=0.16]{images/Figure_nm.jpg}
  \caption{Comparison between different algorithms when $d=k$. The $y$-axis represents 'the number of guessed cards'$-d$. The $95\%$ confidence intervals are highlighted.}\label{fig:CardGuessingM=n}
\end{figure}



\begin{remark}
From this data, the greedy algorithm guesses at least $d$ cards correctly. From previous data, it was not clear if the excess over $k$ even got as large as $2$ (!). We now believe that for $k=d$, the experiment of the greedy strategy is $d + \sqrt{d} + o(\sqrt{d})$ (see Fig. \ref{fig:nMinusSqrtn} ).
\end{remark}

\begin{figure}[htbp]
\begin{center}
  \includegraphics[scale=0.13]{images/nsqrtn.png}
  \caption{The plot of the `guessed cards' $- \sqrt{d}$ when $d=k$. The $95\%$ confidence intervals are  too narrow to present, with $(2.8213, 2.8484)$ for $d=2$ and $(66.5565, 67.2839)$ for $d=62$.}\label{fig:nMinusSqrtn}
\end{center}
\end{figure}



==> sampling matching with importance sampling (Version 12917)/old_intro.tex <==


% main goal
Given a bipartite graph $G(X, Y)$ with $|X|=|Y|=n$, a perfect matching is a subgraph of $G$ in which all vertices have degree exactly one. We study the question of uniform sampling of perfect matchings in bipartite graphs. By the classical equivalences between approximate counting and sampling \cite{JERRUM1986169}, the study of sampling perfect matchings is equivalent to approximating the permanent of the adjacency matrix.

%permanents are hard but people used MCMC
Computing the permanent of an arbitrary $0-1$ matrix is $\#$P-complete \cite{VALIANT1979189}. In fact, the class of $\#$P-complete problems was introduced for the particular problem of computing permanent.
Despite the fact that there seems to be no algorithm for computing the permanent in the general case, when all the entries of the matrix is nonnegative real numbers there exists a fully polynomial randomized approximation scheme (FPRAS) \cite{Jerrum:2004:PAA:1008731.1008738}. This celebrated result is based on Markov Chain Monte Carlo (MCMC) methods where they use a general technique former designed by Broder to analyze the mixing time of an ergodic Markov chain \cite{SINCLAIR198993, Broder1986HowHI}.


% importance sampling as another method
In parallel to MCMC methods, importance sampling is another method to approximate the permanent. Diaconis and Kolesnik \cite{Diaconis2018SequentialIS,diaconis2019randomized}, analyzed an importance sampling algorithm as follows: First draw a uniform permutation $\pi$ over one side of the graph, $X$. Then iterate over the vertices in $X$ according to $\pi$, and in step $i$ match the vertex $\pi(i)$ with one of its neighbor in $Y$ (amongst the remaining allowable options), drawn uniformly at random. Diaconis and Kolesnik \cite{Diaconis2018SequentialIS,diaconis2019randomized} proved central limit theorems for the number of samples when input is Fibonacci permutations, a special case of ``interval" graphs in which the vertex $i$ in $X$ is adjacent to the vertices $[i-s,i+t]$ in $Y$ for some fixed $s, t\geq 0$. In a different work, permanents of more general classes of interval graphs have been studied by Tsao \cite{tsao2020theoretical}. 


%modification of the algorithm
Here, we use a similar algorithm. However, instead of drawing edges uniformly at random, we use the doubly stochastic scaling of the adjacency matrix to draw edges. See Algorithm  \ref{alg: SIS-matching}, which outputs a perfect matching along with the probability of sampling such matching.
We have two main theoretical contributions in this paper. First, we bound the number of samples needed for Algorithm \ref{alg: SIS-matching} to approximate the uniform distribution when the underlying graph is $\lambda$-dense, defined as follows. For some constant $\lambda>0$, the  bipartite graph $G(X,Y)$ with $|X|=|Y|=n$  is called  $\lambda$-dense if the degree of each vertex is at least $(\frac{1}{2}+\lambda)n$. 
Second, we give faster implementation of the algorithm in \cite{diaconis2019randomized} for sampling one perfect matching for general graphs (see Appendix \ref{sec: fast implmnt SIS}).

To state the main result, we need the following notation. For an adjacency matrix $A$, define its doubly-stochastic scaling $Q^A$, a matrix with row and column sums equal to $1$, which can be written as
\begin{equation}\label{eq: DS scaling}
    Q^A=D_\alpha A D_\beta,\qquad \text{$D_\alpha$ and $D_\beta$ are diagonal matrices.}
\end{equation}
 Let $(M_1,X_1),\ldots,(M_N,X_N)$ be the outputs of $N$ independent runs of Algorithm \ref{alg: SIS-matching} with $Q^A$ as an input, where $M_i$ is a perfect matching and $X_i$ is the probability of sampling $M_i$. To count the number of perfect matchings define the estimator as
\begin{equation}\label{eq: matching estimator}
I_N=\frac{1}{N}\sum_{i=1}^NX_i^{-1}.
\end{equation}


\begin{theorem} \label{thm: PTAS dense graph}
Given $\lambda>0$ let $G$ be a $\lambda$-dense graph of size $2n$. Also, let $M(G)$ be the number of perfect matchings in $G$. Then
Algorithm \ref{alg: SIS-matching} with $Q^A$ as an input, is a polynomial time approximation scheme (PTAS) for $M(G)$, i.e, given $\epsilon>0$, there exists a constant $C>0$ such that for $N\geq Cn^{\frac{1-2\lambda}{8\lambda}+\epsilon^{-2}}$, \[\mathbb{E}\left(\frac{|I_N-M(G)|}{M(G)}\right)\leq 3\epsilon.\]
\end{theorem}

%lit. rev. dense
 For a dense bipartite graphs, in which the degree of each vertex is more than $n/2$, Jerrum and Sinclair showed the running time of their algorithm to approximate permanent is $O(n^{10}\log(n)^3)poly\log(\epsilon^{-1})$, where $\epsilon$ is the total variation distance of the uniform distribution and their sampling distribution \cite{Jerrum:2004:PAA:1008731.1008738}. This was improved to $O(n^7\log(n)^4)$ by Bez\'{a}kov\'{a} \cite{bezakova}. Later an exact sampling algorithm for very dense graphs, where the degree of each vertex is at least $\lambda n$ for $\lambda>0.5$, was introduced in \cite{Huber-Law} based on rejection sampling, with the expected running time $O(n^4\log(n))$ for $\lambda\geq 0.6$. Their algorithm iterates over columns of the matrix  and chooses its match using a weaker version of Bregman-Minc inequality \cite{Bregman} to estimate the marginal probability of choosing a certain entry in each column. 

Here, we use the results by Chatterjee and Diaconis \cite{diaconis-chatterjee} to bound the number of samples in sequential importances algorithms. In general,  sequential importance sampling is used to   to approximate a complicated measure $\mu$ with a relatively simple measure $\nu$.
Chatterjee and Diaconis \cite{diaconis-chatterjee} characterized the necessary and sufficient number of samples by the KL-diveregence from $\nu$ to $\mu$, when $\log(d\nu/d\mu)$ is concentrated.  The main ingredient of proof of Theorem \ref{thm: PTAS dense graph} is to bound KL-divergence and use their result to find an upper bound on the number of samples.


\begin{remark}
Theorem \ref{thm: PTAS dense graph} bounds the number of samples needed by Algorithm \ref{alg: SIS-matching} with $Q^A$ as an input to approximate the number of perfect matchings in a $\lambda$-dense graph. Appendix \ref{sec:counter example matching} gives an example of graph with a bounded average degree that the original method of choosing edges uniformly at random in \cite{diaconis2019randomized} needs exponential number of samples, while using the doubly stochastic scaling will only need linear number of samples.
\end{remark}

Finally, we apply our algorithm to implement the greedy algorithm in card guessing experiments: A deck of $n$ cards is shuffled and then we have to guess the card on top of the deck sequentially. After each guess, we are told either our guess is wrong or right. Greedy algorithm is to guess most likely card at each step. While this algorithm is not optimal, it is known to be close to optimal. See \cite{diaconis2020card,diaconis2020guessing} for recent results on this topic.

Implementation of greedy needs approximating permanent of dense matrices repeatedly,for which we use Algorithm \ref{alg: SIS-matching}. Whereas the previous results could only approximate greedy for small decks, we are now able to apply the computations for decks of size $400$ (Figure \ref{fig:CardGuessingM=n}). 

%TODO add the latin square here

\subsection{Overview of the paper}
We start by going over some preliminaries on importance sampling in Section \ref{sec: prelim IS}. Then we proceed by proving Theorem \ref{thm: PTAS dense graph} in Section \ref{sec:dense}. The main idea is to bound the KL-divergence of the sampling distribution of Algorithm \ref{alg: SIS-matching}  with respect to the uniform distribution over the set of perfect matchings when the input matrix of the algorithm is the doubly stochastic scaling of the adjacency matrix.  Sections \ref{sec: experiment} and \ref{sec: latin square} is on the applications of our result to card guessing games and counting the number of Latin squares, respectively. 
